Domain-Adaptive Pre-Training for Arabic Aspect-Based Sentiment Analysis: A Comparative Study of Domain Adaptation and Fine-Tuning Strategies

Aspect-based sentiment analysis (ABSA) in natural language processing enables organizations to understand customer opinions on specific product aspects. While deep learning models are widely used for English ABSA, their application in Arabic is limited due to the scarcity of labeled data. Researchers have attempted to tackle this issue by using pre-trained contextualized language models such as BERT. However, these models are often based on fact-based data, which can introduce bias in domain-specific tasks like ABSA. To our knowledge, no studies have applied adaptive pre-training with Arabic contextualized models for ABSA. This research proposes a novel approach using domain-adaptive pre-training for aspect-sentiment classification (ASC) and opinion target expression (OTE) extraction. We examine fine-tuning strategies - feature extraction, full fine-tuning, and adapter-based methods - to enhance performance and efficiency, utilizing multiple adaptation corpora and contextualized models. Our results show that in-domain adaptive pre-training yields modest improvements. Adapter-based fine-tuning is a computationally efficient method that achieves competitive results. However, error analyses reveal issues with model predictions and dataset labeling. In ASC, common problems include incorrect sentiment labeling, misinterpretation of contrastive markers, positivity bias for early terms, and challenges with conflicting opinions and subword tokenization. For OTE, issues involve mislabeling targets, confusion over syntactic roles, difficulty with multi-word expressions, and reliance on shallow heuristics. These findings underscore the need for syntax- and semantics-aware models, such as graph convolutional networks, to more effectively capture long-distance relations and complex aspect-based opinion alignments.

==> ACSA.tex <==
\begin{table}[htp!]
\centering
\caption{Accuracy of models for Aspect Category Sentiment Classification (ACSC) on various English datasets. The dataset IDs (ED) refer to English dataset identifiers defined in Table~\ref{tab:SemEval2014DS} and Table~\ref{tab:SemEval20152016TL}. Bold indicates the highest scores.}
\label{tab:EN_ACSC_LR}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Ref} & \textbf{Year} & \textbf{Dataset ID} & \textbf{Model} & \textbf{Word Embedding} & \textbf{Accuracy (\%)} \\ \hline
\cite{Tang2016b} & 2015 & ED1 & TD-LSTM & GloVe 300D & 82.6 \\ \hline
\cite{Tang2016b} & 2015 & ED1 & TC-LSTM & GloVe 300D & 81.9 \\ \hline
\cite{Wang2016c} & 2016 & ED1 & ATAE-LSTM & GloVe 300D & 84.0 \\ \hline
\cite{sun-etal-2019-utilizing} & 2019 & ED1 & \begin{tabular}[c]{@{}c@{}}BERT-pair-\\ QA-B\end{tabular} & BERT & \textbf{89.9} \\ \hline
\cite{scaria2023instructabsa} & 2023 & ED5 & InstructABSA2 & Tk-Instruct & 89.43 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> AROTELR.tex <==
\begin{table}[htp!]
\centering
\caption{Summary of \gls{ote} extraction techniques for Arabic \gls{absa}. All techniques listed are explicit \gls{ote}s. N/A = not available, TF = term frequency, TF-IDF = term frequency-inverse document frequency, \gls{pos} = part-of-speech, \gls{ner} = named-entity recognition. Best results are in \textbf{bold}.}

\label{tab:ArabicOTEExtractionTechniques}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Reference} & \textbf{Technique} & \textbf{Word Representation} & \textbf{F1-Score (\%)} \\ \hline
\multicolumn{4}{|c|}{\textbf{Israel-Gaza 2014 Conflict Breaking News Posts Dataset}} \\ \hline
\citep{Bensoltane2022_S50} & \gls{bert}-\gls{bi-gru}-\gls{crf} & Ara\gls{bert} & \textbf{88.1} \\ \hline
\multicolumn{4}{|c|}{\textbf{Arabic Hotels Reviews-2016}} \\ \hline
\citep{ALSMADI2018_S23} & \gls{rnn}-Softmax & \begin{tabular}[c]{@{}c@{}}\gls{word2vec}, N-grams,\\ \gls{pos} tags, \gls{ner}, TF, TF-IDF\end{tabular} & 48 \\ \hline
\citep{Al-Smadi2019c_S30} & \gls{bi-lstm}-\gls{crf} & fastText & 69.98 \\ \hline
\citep{Al-Dabet2020a_S41} & \begin{tabular}[c]{@{}c@{}}Encoder (\gls{cnn}-\gls{bi-lstm})\\ Attention Decoder (\gls{lstm}-\gls{crf})\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pretrained \gls{word2vec},\\ \gls{cnn}-character embedding\end{tabular} & 72.83 \\ \hline
\citep{Abdelgwad2021_S47} & \gls{cnn}-\gls{bi-gru}-\gls{crf} & \begin{tabular}[c]{@{}c@{}}fastText,\\ \gls{cnn}-character embedding\end{tabular} & 70.67 \\ \hline
\citep{Fadel2022} & \begin{tabular}[c]{@{}c@{}}Flair + Ara\gls{bert} Stacked\\ Embeddings \gls{bi-lstm}-\gls{crf}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Ara\gls{bert} +\\ Arabic Flair embedding\end{tabular} & \textbf{79.7} \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> ASCENRESTTL.tex <==
\begin{table}[htp!]
\centering
\caption{Summary of Aspect-Term Sentiment Analysis Techniques on SemEval-2014 English Restaurant Reviews. Bold indicates the highest scores. Gains from domain adaptation are shown as percentages in parentheses. "N/A" indicates data not available.}
\label{tab:ASCtermEN_RES2014}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Reference} & \textbf{Year} & \textbf{Model} & \textbf{Word Embedding} & \textbf{Macro-F1 (\%)} & \textbf{Accuracy (\%)} \\ \hline
\cite{Tang2016b} & 2015 & TD-LSTM & Pretrained 300D-Glove & N/A & 75.6 \\ \hline
\multicolumn{6}{|c|}{\textbf{LSTM+Attention}} \\ \hline
\cite{Wang2016c} & 2016 & ATAE-LSTM & Pretrained 300D-Glove & N/A & 77.2 \\ \hline
\cite{He2018} & 2018 & \begin{tabular}[c]{@{}c@{}}LSTM + SynATT\\ + TarRep\end{tabular} & Pretrained 300D-Glove & 71.32 & 80.63 \\ \hline
\multicolumn{6}{|c|}{\textbf{Interactive Attention LSTM}} \\ \hline
\cite{Ma2017} & 2017 & IAN & Pretrained 300D-Glove & N/A & 78.6 \\ \hline
\cite{Huang2018} & 2018 & AOA-LSTM & Pretrained 300D-Glove & N/A & 81.2 \\ \hline
\cite{Fan2020} & 2018 & MGAN & Pretrained 300D-Glove & 71.94 & 81.25 \\ \hline
\multicolumn{6}{|c|}{\textbf{Memory-Based}} \\ \hline
\cite{Tang2014a} & 2016 & MemNet & Pretrained 300D-Glove & N/A & 80.95 \\ \hline
\cite{chen-etal-2017-recurrent} & 2017 & RAM & Pretrained 300D-Glove & 70.80 & 80.23 \\ \hline
\multicolumn{6}{|c|}{\textbf{CNN}} \\ \hline
\cite{Kumar2020} & 2020 & IGCN & \begin{tabular}[c]{@{}c@{}}Domain-specific 100D-Fasttext +\\ POS + position\end{tabular} & N/A & 81.34 \\ \hline
\cite{Ruidan2019} & 2019 & IMN & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove +\\ Domain-specific 100D-Fasttext\end{tabular} & 75.66 & 83.89 \\ \hline
\multicolumn{6}{|c|}{\textbf{BERT with Domain Adaptation}} \\ \hline
\cite{Xu2019} & 2019 & BERT-DK & Dom+BERT & 75.45 & 83.96 (+2.92) \\ \hline
\cite{Xu2019} & 2019 & PT-BERT & Dom+BERT & 76.96 & 84.95 \\ \hline
\cite{Xu2020c} & 2020 & DomBERT & Dom+BERT & 75.00 & 83.14 (+1.6) \\ \hline
\cite{Rietzler2020} & 2019 & BERT-ADA Joint & Dom+BERT & 81.20 & 87.69 (+3.6) \\ \hline
\cite{YANG2021344} & 2020 & LCF-ATEPC-Fusion & Dom+BERT & 84.76 & \textbf{89.45 (+2.68)} \\ \hline
\multicolumn{6}{|c|}{\textbf{BERT without Domain Adaptation}} \\ \hline
\cite{Song2019c} & 2019 & AEN-BERT & BERT & 73.76 & 83.12 \\ \hline
\cite{Song2019c} & 2019 & BERT-SPC & BERT & 76.98 & 84.46 \\ \hline
\cite{Zhaoa2019} & 2019 & SDGCN-BERT & BERT & 76.47 & 83.57 \\ \hline
\cite{Zeng_lcf_first} & 2019 & LCF-BERT Glo-CDW & BERT & 81.74 & 87.14 \\ \hline
\cite{YANG2021344} & 2020 & LCF-ATEPC-Fusion & BERT & 80.54 & 86.77 \\ \hline
\cite{ABSALSA} & 2022 & LSAT-BERT & BERT & 81.86 & 87.32 \\ \hline
\cite{ABSALSA} & 2022 & LSAT-DeBERTa & DeBERTa & 85.05 & \textbf{89.91} \\ \hline
\cite{ABSALSA} & 2022 & LSAT-RoBERTa & RoBERTa & 83.09 & 88.30 \\ \hline
\multicolumn{6}{|c|}{\textbf{Instruction-Tuning}} \\ \hline
\cite{scaria2023instructabsa} & 2023 & InstructABSA1 & Tk-Instruct & N/A & 86.25 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> ASCENTL.tex <==
\begin{table}[htp!]
\centering
\caption{Summary of Aspect-Term Sentiment Analysis Techniques on SemEval-2014 English Laptop Reviews. Bold indicates the highest scores. Gains from domain adaptation are shown as percentages in parentheses. "N/A" indicates data not available.}
\label{tab:ASCtermEN_LAP2014}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Reference} & \textbf{Year} & \textbf{Model} & \textbf{Word Embedding} & \textbf{Macro-F1 (\%)} & \textbf{Accuracy (\%)} \\ \hline
\cite{Tang2016b} & 2015 & TD-LSTM & Pretrained 300D-Glove & N/A & 68.1 \\ \hline
\multicolumn{6}{|c|}{\textbf{LSTM+Attention}} \\ \hline
\cite{Wang2016c} & 2016 & ATAE-LSTM & Pretrained 300D-Glove & N/A & 68.7 \\ \hline
\cite{He2018} & 2018 & \begin{tabular}[c]{@{}c@{}}LSTM + SynATT\\ + TarRep\end{tabular} & Pretrained 300D-Glove & 69.23 & 71.94 \\ \hline
\multicolumn{6}{|c|}{\textbf{Interactive Attention LSTM}} \\ \hline
\cite{Ma2017} & 2017 & IAN & Pretrained 300D-Glove & N/A & 72.1 \\ \hline
\cite{Huang2018} & 2018 & AOA-LSTM & Pretrained 300D-Glove & N/A & 74.5 \\ \hline
\cite{Fan2020} & 2018 & MGAN & Pretrained 300D-Glove & 72.4 & 75.39 \\ \hline
\multicolumn{6}{|c|}{\textbf{Memory-Based}} \\ \hline
\cite{Tang2014a} & 2016 & MemNet & Pretrained 300D-Glove & N/A & 72.21 \\ \hline
\cite{chen-etal-2017-recurrent} & 2017 & RAM & Pretrained 300D-Glove & 71.35 & 74.49 \\ \hline
\multicolumn{6}{|c|}{\textbf{CNN}} \\ \hline
\cite{Kumar2020} & 2020 & IGCN & \begin{tabular}[c]{@{}c@{}}Domain-specific\\ 100D-Fasttext +\\ POS + position\end{tabular} & N/A & 75.24 \\ \hline
\cite{Ruidan2019} & 2019 & IMN & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove +\\ Domain-specific 100D-Fasttext\end{tabular} & 72.02 & 75.36 \\ \hline
\multicolumn{6}{|c|}{\textbf{BERT with Domain Adaptation}} \\ \hline
\cite{Xu2019} & 2019 & BERT-DK & Dom+BERT & 73.72 & 77.01 (+6.85) \\ \hline
\cite{Xu2019} & 2019 & PT-BERT & Dom+BERT & 75.08 & 78.07 \\ \hline
\cite{Xu2020c} & 2020 & DomBERT & Dom+BERT & 73.46 & 76.72 (+1.43) \\ \hline
\cite{Rietzler2020} & 2019 & BERT-ADA Joint & Dom+BERT & 78.74 & 79.94 (+2.2) \\ \hline
\cite{YANG2021344} & 2020 & LCF-ATEPC-Fusion & Dom+BERT & 78.65 & 81.76 (+0.79) \\ \hline
\multicolumn{6}{|c|}{\textbf{BERT without Domain Adaptation}} \\ \hline
\cite{Song2019c} & 2019 & AEN-BERT & BERT & 76.31 & 79.93 \\ \hline
\cite{Song2019c} & 2019 & BERT-SPC & BERT & 75.03 & 78.99 \\ \hline
\cite{Zhaoa2019} & 2019 & SDGCN-BERT & BERT & 78.34 & 81.35 \\ \hline
\cite{Zeng_lcf_first} & 2019 & LCF-BERT Glo-CDW & BERT & 79.59 & 82.45 \\ \hline
\cite{YANG2021344} & 2020 & LCF-ATEPC-Fusion & BERT & 77.86 & 80.97 \\ \hline
\cite{ABSALSA} & 2022 & LSAT-BERT & BERT & 78.43 & 81.35 \\ \hline
\cite{ABSALSA} & 2022 & LSAT-DeBERTa & DeBERTa & 82.00 & \textbf{84.80} \\ \hline
\cite{ABSALSA} & 2022 & LSAT-RoBERTa & RoBERTa & 80.47 & 83.44 \\ \hline
\multicolumn{6}{|c|}{\textbf{Instruction-Tuning}} \\ \hline
\cite{scaria2023instructabsa} & 2023 & InstructABSA2 & Tk-Instruct & N/A & 81.56 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> ArabicABSADSExamples.tex <==
\begin{longtable}{|c|c|}
\caption{Arabic ABSA datasets Examples} \label{table:ArabicDatasetsExamples} \\

\hline \textbf{Ref} & \textbf{Example} \\ \hline
\endfirsthead

\multicolumn{2}{c}%
{{\bfseries Table \thetable\ Arabic ABSA datasets Examples Continued}} \\
\hline \textbf{Ref} & \textbf{Example} \\ \hline
\endhead

\hline \multicolumn{2}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

\cite{Al_Smadi_2015_S5} & \includegraphics[width=0.8\textwidth]{FCITThesisTemplate(V7)/img_chapter2/HAAD_EX.jpeg} \\ \hline
\cite{AL-Smadi_2016_S17} & \includegraphics[width=0.8\textwidth]{FCITThesisTemplate(V7)/img_chapter2/Semeval_hotel_ex.jpeg} \\ \hline
\cite{Al-Ayyoub_2017_S24} & \includegraphics[width=0.8\textwidth]{FCITThesisTemplate(V7)/img_chapter2/laptopReview.jpeg} \\ \hline
\cite{Al_Sarhan_2016_S16} & \includegraphics[width=0.8\textwidth]{FCITThesisTemplate(V7)/img_chapter2/Gaza_conflict.jpeg} \\ \hline

\end{longtable}

==> ArabicABSAdatasets.tex <==
\begin{table*}[htp!]
\centering
\caption{Summary of the public Arabic ABSA datasets. MSA: Modern Standard Arabic, DA: Dialectal Arabic, OTE: Opinion Target Expression, E\#A: Entity\#Attribute.}
\label{table:ArabicDatasets}
\begin{minipage}{\textwidth}
\setcounter{mpFootnoteValueSaver}{\value{footnote}}
\setlength{\tabcolsep}{2pt}
\Large
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset Name (Reference)} & \textbf{Arabic Language Type} & \textbf{Annotated ABSA Tasks} & \textbf{Domain} & \textbf{Size} & \textbf{Balanced} & \textbf{ID} \\ \hline
\begin{tabular}[c]{@{}c@{}}HAAD book\\ reviews\\ \citep{Al_Smadi_2015_S5}\\ \footnote{\url{https://github.com/msmadi/HAAD/tree/master/Dataset}}\end{tabular} & Arabic (MSA and DA) & \begin{tabular}[c]{@{}c@{}}Aspect term,\\ Aspect term\\ polarity,\\ Aspect category,\\ Aspect category\\ polarity\end{tabular} & Book & \begin{tabular}[c]{@{}c@{}}1513 sentences,\\ OTE: 2838\\ (1296 distinct),\\ Aspect category: 14\end{tabular} & No & D1 \\ \hline
\begin{tabular}[c]{@{}c@{}}Israel-Gaza 2014\\ conflict breaking\\ news posts\\ \citep{Al_Sarhan_2016_S16}\\ \footnote{\url{https://github.com/malayyoub/ABSA-for-Affective-News-Analysis-}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Posts: Arabic\\ (MSA)\\ Comments: Arabic\\ (MSA and DA)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Posts: Aspect term,\\ Aspect term\\ polarity,\\ Aspect category,\\ Aspect category\\ polarity\\ Comments: Aspect\\ category,\\ Aspect category\\ polarity\end{tabular} & News & \begin{tabular}[c]{@{}c@{}}Posts: 2265\\ posts, Aspect\\ term: 9655,\\ Aspect category: 4\\ Comments: 13628\\ comments,\\ Aspect category: 5\end{tabular} & No & D2 \\ \hline
\begin{tabular}[c]{@{}c@{}}SemEval-2016\\ Arabic hotel\\ reviews\\ \citep{AL-Smadi_2016_S17}\\ \footnote{\url{https://github.com/msmadi/ABSA-Hotels}}\end{tabular} & Arabic (MSA and DA) & \begin{tabular}[c]{@{}c@{}}Sentence level:\\ Aspect category\\ \{E/\#A\},\\ Explicit OTE,\\ Aspect category\\ polarity\\ Document level:\\ Aspect category\\ \{E/\#A\},\\ Aspect category\\ polarity\end{tabular} & Hotel & \begin{tabular}[c]{@{}c@{}}Sentence Level:\\ 6029 sentences,\\ 13133 \{E/\#A,\\ OTE, Polarity\}\\ tuples\\ Document Level:\\ 2291 Reviews,\\ 10915 \{E/\#A,\\ OTE, Polarity\}\\ tuples\end{tabular} & No & D3 \\ \hline
\begin{tabular}[c]{@{}c@{}}Arabic-Laptop-\\ Reviews\\ \citep{Al-Ayyoub_2017_S24}\\ \footnote{\url{https://github.com/bashartalafha/Arabic-Laptop-Reviews-ALR-Dataset}}\end{tabular} & Arabic (MSA and DA) & \begin{tabular}[c]{@{}c@{}}Sentence level:\\ Aspect category\\ \{E/\#A\},\\ Aspect category\\ polarity\end{tabular} & Laptop & \begin{tabular}[c]{@{}c@{}}1028 reviews,\\ 1753 sentences,\\ 131 \{E/\#A,\\ Polarity\} tuples\end{tabular} & No & D4 \\ \hline
\end{tabular}
\end{adjustbox}
\end{minipage}
\end{table*}




==> ArabicASCLR.tex <==
\begin{table*}[htp!]
\centering
\caption{Summary of aspect sentiment classification techniques for Arabic text. 'Aspect category' includes both implicit and explicit aspects, while 'Aspect category for explicit \gls{ote}s' focuses on explicit aspects. N/A = not available, \gls{tf} = term frequency, \gls{tfidf} = term frequency-inverse document frequency, \gls{pos} = part-of-speech, \gls{ner} = named-entity recognition. Best results are in \textbf{bold}.}
\label{tab:ASCArabicTechniques}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Reference} & \textbf{Aspect Level} & \textbf{Technique} & \textbf{Word Representation} & \multicolumn{2}{c|}{\textbf{Performance (\%)}} \\ \hline
 &  &  &  & \textbf{Macro-F1} & \textbf{Accuracy} \\ \hline
\multicolumn{6}{|c|}{\textbf{\gls{haad} Book Review}} \\ \hline
\citep{Abdelgwad2022} & Aspect term & SP-Arabic \gls{bert} & Sentence and opinion target term Arabic \gls{bert} & N/A & 73.23 \\ \hline
\multicolumn{6}{|c|}{\textbf{Israel-Gaza 2014 Conflict Breaking News Posts}} \\ \hline
\citep{Abdelgwad2022} & Aspect term & SP-Arabic \gls{bert} & Sentence and opinion target term Arabic \gls{bert} & N/A & 85.73 \\ \hline
\multicolumn{6}{|c|}{\textbf{Arabic Hotels Reviews \gls{semeval}-2016}} \\ \hline
\citep{ALSMADI2018_S23} & Aspect category & \gls{rnn} & \begin{tabular}[c]{@{}c@{}}\gls{word2vec}, N-grams,\\ \gls{pos} tags, \gls{ner}, \gls{tf}, \gls{tfidf}\end{tabular} & N/A & 87 \\ \hline
\citep{ruder-etal-2016-insight-1_S12} & \begin{tabular}[c]{@{}c@{}}Aspect category\\ for explicit \gls{ote}s\end{tabular} & \gls{cnn} & \begin{tabular}[c]{@{}c@{}}Aspect category embedding,\\ word embedding\end{tabular} & N/A & 82.72 \\ \hline
\citep{ruder-etal-2016-hierarchical_S14} & \begin{tabular}[c]{@{}c@{}}Aspect category\\ for explicit \gls{ote}s\end{tabular} & Multi-layer \gls{bi-lstm} & \begin{tabular}[c]{@{}c@{}}Pretrained \gls{word2vec},\\ aspect category embedding\end{tabular} & N/A & 82.90 \\ \hline
\citep{Liu_S42} & \begin{tabular}[c]{@{}c@{}}Aspect category\\ for explicit \gls{ote}s\end{tabular} & \begin{tabular}[c]{@{}c@{}}\gls{cnn}-Multi-layer \gls{bi-lstm}\\ and \gls{rcnn}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pretrained \gls{word2vec},\\ \gls{cnn} character-level embedding\end{tabular} & 86.89 & 86.87 \\ \hline
\citep{Wang_Lu_2018_S32} & \begin{tabular}[c]{@{}c@{}}Aspect category\\ for explicit \gls{ote}s\end{tabular} & \gls{bi-lstm}-Segment attention & \begin{tabular}[c]{@{}c@{}}Pretrained \gls{word2vec} embedding,\\ binary \gls{ote} indicator\end{tabular} & N/A & 86.90 \\ \hline
\citep{Al-Smadi2019c_S30} & \begin{tabular}[c]{@{}c@{}}Aspect category\\ for explicit \gls{ote}s\end{tabular} & \gls{bi-lstm}-Soft attention & \begin{tabular}[c]{@{}c@{}}\gls{word2vec},\\ \gls{ote} embedding\end{tabular} & N/A & 82.60 \\ \hline
\citep{Abdelgwad2021_S47} & \begin{tabular}[c]{@{}c@{}}Aspect category\\ for explicit \gls{ote}s\end{tabular} & \gls{cnn}-\gls{bi-gru}-Interactive attention & \begin{tabular}[c]{@{}c@{}}Pretrained \gls{word2vec},\\ \gls{ote} embedding\end{tabular} & N/A & 83.98 \\ \hline
\citep{Al-Dabet_2021_S48} & \begin{tabular}[c]{@{}c@{}}Aspect category\\ for explicit \gls{ote}s\end{tabular} & \begin{tabular}[c]{@{}c@{}}Memory network (\gls{indylstm}s),\\ recurrent attention\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pretrained fastText,\\ sentiment feature\end{tabular} & N/A & 87.31 \\ \hline
\citep{Almani2019_S35} & \begin{tabular}[c]{@{}c@{}}Aspect category\\ for explicit \gls{ote}s\end{tabular} & \gls{gru}-Self attention & \begin{tabular}[c]{@{}c@{}}Pretrained \gls{word2vec},\\ \gls{ote} embedding\end{tabular} & 76 & 77 \\ \hline
\citep{Abdelgwad2022} & \begin{tabular}[c]{@{}c@{}}Aspect category\\ for explicit \gls{ote}s\end{tabular} & SP-Arabic \gls{bert} & \begin{tabular}[c]{@{}c@{}}Sentence and opinion\\ target term Arabic \gls{bert}\end{tabular} & N/A & \textbf{89.51} \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}


==> BestHyperparamterAndModelsTL.tex <==
\begin{table}[htp!]
\centering
\caption{Performance metrics for selected pre-trained models using different fine-tuning techniques for two different tasks: Opinion Target Extraction (OTE) and Aspect Sentiment Classification (ASC). The best results are highlighted in \textbf{bold}.}
\label{tab:SELECTED_MODELS}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Pretrained Model} & \textbf{Fine-Tuning Technique} & \textbf{Task} & \textbf{Learning Rate} & \textbf{Batch Size} & \textbf{\# of Epochs} & \textbf{Micro-F1 (\%)} & \textbf{Accuracy (\%)} \\ \hline
MARBERTv2 & Full & OTE & $2.00 \times 10^{-6}$ & 32 & 25 & \textbf{76.92} & N/A \\ \hline
MARBERTv2 & Feature Extraction & OTE & $9.4 \times 10^{-3}$ & 32 & 10 & 69.36 & N/A \\ \hline
CAMeLBERT-MSA & Full & OTE & $5.00 \times 10^{-5}$ & 32 & 10 & 76.69 & N/A \\ \hline
CAMeLBERT-MSA & Feature Extraction & OTE & $0.002$ & 32 & 5 & 70.55 & N/A \\ \hline
QARiB & Full & OTE & $5.00 \times 10^{-5}$ & 32 & 5 & 76.68 & N/A \\ \hline
QARiB & Feature Extraction & OTE & $0.002$ & 32 & 10 & 70.95 & N/A \\ \hline
MARBERTv2 & Full & ASC & $2.00 \times 10^{-6}$ & 32 & 25 & N/A & \textbf{87.35} \\ \hline
MARBERTv2 & Feature Extraction & ASC & $9.4 \times 10^{-3}$ & 32 & 10 & N/A & 83.91 \\ \hline
CAMeLBERT-MSA & Full & ASC & $5.00 \times 10^{-5}$ & 32 & 5 & N/A & 86.91 \\ \hline
CAMeLBERT-MSA & Feature Extraction & ASC & $0.0094$ & 32 & 10 & N/A & 84.29 \\ \hline
QARiB & Full & ASC & $5.00 \times 10^{-5}$ & 32 & 5 & N/A & 87.25 \\ \hline
QARiB & Feature Extraction & ASC & $0.0094$ & 32 & 10 & N/A & 85.31 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> DomainCorpusSizeTL.tex <==
\begin{table}[htp!]
\centering
\caption{Corpus sizes used for domain adaptation in English studies.}
\label{tab:corpusSize}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Ref} & \textbf{Domain Corpus} & \textbf{Domain Corpus Size} \\ \hline
\multirow{3}{*}{\cite{Xu2019}} & Yelp restaurant reviews & 700,000 Examples \\ \cline{2-3}
                               & Amazon laptop reviews & 230,373 Examples \\ \cline{2-3}
                               & SQuAD 1.1 & 87,599 Examples \\ \hline
\multirow{3}{*}{\cite{Xu2020c}} & Yelp restaurant reviews & 100 MB \\ \cline{2-3}
                                & Amazon laptop reviews & 100 MB \\ \cline{2-3}
                                & \begin{tabular}[c]{@{}c@{}}Other domains from Yelp \\ and Amazon datasets\end{tabular} & 19.8 GB \\ \hline
\multirow{3}{*}{\cite{Rietzler2020}} & Yelp restaurant reviews & 1,007,209 \\ \cline{2-3}
                                     & Amazon laptop reviews & 10,000,000 \\ \cline{2-3}
                                     & Joint restaurant + laptop & 2,007,213 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> ENABSADataset.tex <==
\begin{table}[htp!]
\centering
\caption{Summary of SemEval-2015 and SemEval-2016 Laptop and Restaurant English Datasets.}
\label{tab:SemEval20152016TL}
\begin{adjustbox}{ width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Dataset} &
  \multirow{2}{*}{Format} &
  \multirow{2}{*}{Training} &
  \multirow{2}{*}{Testing} &
  \multirow{2}{*}{Total} &
  \multicolumn{3}{c|}{Tuples} &
  \multirow{2}{*}{Balanced} & \multirow{2}{*}{ID}  \\ \cline{6-8}
 &
   &
   &
   &
   &
  Format &
  Train &
  Test & &
   \\ \hline
\begin{tabular}[c]{@{}c@{}}Laptop Reviews\\ -2015\\ \cite{Pontiki2015}\end{tabular} &
  SemEval-2015 &
  \begin{tabular}[c]{@{}c@{}}1739\\ Sentences,\\ 277 Reviews\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}761\\ Sentences\end{tabular} &
  2,500 &
  \{E\#A, polarity\} &
  1974 &
  949 &
  No & ED3 \\ \hline
\begin{tabular}[c]{@{}c@{}}Restaurant Reviews\\ -2015\\ \cite{Pontiki2015}\end{tabular} &
  SemEval-2015 &
  \begin{tabular}[c]{@{}c@{}}1315\\ Sentences\\ 254\\ Reviews\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}685\\ Sentences\end{tabular} &
  2,000 &
  \{E\#A, OTE, polarity\} &
  1654 &
  845 &
  No & ED4 \\ \hline
\begin{tabular}[c]{@{}c@{}}Restaurant Reviews\\ 2016-SB1\\ \cite{SemEval2016}\end{tabular} &
  SemEval-2016 &
  \begin{tabular}[c]{@{}c@{}}2000\\ Sentences\\ 350\\ Reviews\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}676\\ Sentences\end{tabular} &
  2676 &
  \{E\#A, OTE, polarity\} &
  2507 &
  859 &
  No & ED5 \\ \hline
\begin{tabular}[c]{@{}c@{}}Restaurant Reviews\\ 2016-SB2\\ \cite{SemEval2016}\end{tabular} &
  SemEval-2016 &
  \begin{tabular}[c]{@{}c@{}}1950\\ Sentences\\ 335 Reviews\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}676\\ Sentences\\ 90\\ Reviews\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}2,626\\ Sentences\\ 425\\ Reviews\end{tabular} &
  \{cat, pol\} &
  1435 &
  404 &
  No & ED6 \\ \hline
\begin{tabular}[c]{@{}c@{}}Laptop Reviews\\ 2016-SB1\\ \cite{SemEval2016}\end{tabular} &
  SemEval-2016 &
  \begin{tabular}[c]{@{}c@{}}2500\\ Sentences\\ 450\\ Reviews\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}808\\ Sentences\\ 80\\ Reviews\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}3,308\\ Sentences\end{tabular} &
  \{E\#A, polarity\} &
  2909 &
  801 &
  No & ED7 \\ \hline
\begin{tabular}[c]{@{}c@{}}Laptop Reviews\\ 2016-SB2\\ \cite{SemEval2016}\end{tabular} &
  SemEval-2016 &
  \begin{tabular}[c]{@{}c@{}}2375\\ Sentences\\ 395\\ Reviews\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}808\\ Sentences\\ 80\\ Reviews\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}3,183\\ Sentences\\ 475\\ Reviews\end{tabular} &
  \{cat, pol\} &
  2082 &
  545 &
  No & ED8 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> ENOTEREST2014TL.tex <==
\begin{table}[htp!]
\centering
\caption{Summary of Opinion Target Extraction Techniques on SemEval-2014 English Restaurant Reviews. Bold indicates the highest scores. Gains from domain adaptation are shown as percentages in parentheses (e.g., "\%1"). "N/A" indicates data not available.}
\label{tab:OTE_EN_RES2014}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Reference} & \textbf{Year} & \textbf{Model} & \textbf{Word Embedding} & \textbf{Performance F1 (\%)} \\ \hline
\multicolumn{5}{|c|}{\textbf{LSTM+Attention}} \\ \hline
\cite{ZschornackRodriguesSaraiva2021} & 2020 & \begin{tabular}[c]{@{}c@{}}POS-AttWD-BLSTM-CRF\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove\end{tabular} & 87.86 \\ \hline
\cite{Li2018} & 2018 & \begin{tabular}[c]{@{}c@{}}THA-STN LSTMs\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove\end{tabular} & 85.61 \\ \hline
\multicolumn{5}{|c|}{\textbf{CNN}} \\ \hline
\cite{Ruidan2019} & 2019 & IMN & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove +\\ Domain-specific 100D-Fasttext\end{tabular} & 83.33 \\ \hline
\multicolumn{5}{|c|}{\textbf{BERT with Domain Adaptation}} \\ \hline
\cite{YANG2021344} & 2020 & LCF-ATEPC-Fusion & Dom+BERT & 89.94 (+0.92) \\ \hline
\multicolumn{5}{|c|}{\textbf{BERT without Domain Adaptation}} \\ \hline
\cite{YANG2021344} & 2020 & LCF-ATEPC-Fusion & BERT & 89.02 \\ \hline
\cite{YANG2021344} & 2020 & LCF-ATE-CDM & BERT & 89.53 \\ \hline
\multicolumn{5}{|c|}{\textbf{Instruction-Tuning}} \\ \hline
\cite{scaria2023instructabsa} & 2023 & InstructABSA1 & Tk-Instruct & \textbf{92.76} \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> ExpermintsandResults.tex <==
\section{Expermints and Results}
\label{sec:ExpermintsAndResults}
\section{Dataset}
We employed two types of datasets: unlabeled datasets for domain and task-adaptive pre-training, and labeled end-task datasets for fine-tuning and evaluating our models. The end tasks included aspect-based sentiment classification (\gls{asc}) and opinion target expression (\gls{ote}) extraction.

\subsection{Domain Adaptation Data}

For adaptive pre-training, we leveraged reviews from the unbalanced version of the \gls{hard} dataset\footnote{\url{https://github.com/elnagara/HARD-Arabic-Dataset}}~\citep{Elnagar2018HotelAD} and the \gls{labr} dataset\footnote{\url{https://github.com/mohamedadaly/LABR}}~\citep{aly-atiya-2013-labr}, both for in-domain (\gls{indapt}) and out-of-domain (\gls{outdapt}) training. Additionally, we used the training portion of the \gls{semeval}-2016 hotel review dataset for task-specific adaptive pre-training (\gls{tapt}).

\subsubsection{Domain Adaptation Data Preprocessing}

During our experiments with domain adaptation data, we applied several preprocessing techniques commonly used by Arabic pre-trained models such as CAMeLBERT \cite{inoue-etal-2021-CAMELBERT} and AraBERT \cite{antoun-etal-2020-arabert}. These techniques included removing extra white spaces, discretization, control characters, and elongation (kashida). We also replaced URLs and user mentions with "URL" and "USER" strings, respectively.

After selecting the top three models with the best performance in the two tasks, we implemented the specific preprocessing steps for each model. The statistics and preprocessing steps for each dataset are provided in Tables \ref{tab:DA Data} and \ref{tab:DAPrep}. Additionally, Figures \ref{fig:DialectsCount} and \ref{fig:OverlapDSMODEL} illustrate the dialect distributions and vocabulary overlap between the datasets, respectively.


\input{DA_DataTL}
\input{DADataPrep}

\subsection{End-Task Datasets}

We evaluated our proposed model using the \gls{semeval}-2016 hotel review dataset \citep{Al-Smadi_2016_S7} to perform \gls{ote} extraction and \gls{asc} tasks. This dataset was created for the \gls{semeval} 2016 competition to assess models on Arabic text. It was derived from \citep{ElSahar2015} and adapted for various \gls{absa} tasks, based on the guidelines from \gls{semeval} 2016 task 5 for sentence-level and text-level tasks. In our research, we specifically utilized the dataset designed for sentence-level tasks.

\subsubsection{End-Task Data Preprocessing}

We converted the \gls{semeval} dataset from XML to CSV format using scripts provided by \footnote{\url{https://github.com/howardhsu/ABSA_preprocessing}}~\citep{Xu2019}. For the \gls{ote} extraction, we labeled each word as "O" if it was not part of the \gls{ote}, "B-\gls{ote}" if it was the beginning of the \gls{ote}, and "I-\gls{ote}" for any word that was part of the \gls{ote} after the start. In terms of aspect categories, we replaced the hashtag (\#) sign with a space between entity and attribute pairs and then normalized them to lowercase. For example, "ROOMS\#GENERAL" became "rooms general". We then followed the same pre-processing steps used for the initial model evaluation, including removing extra white spaces, discretization, control characters, and elongation (kashida). Additionally, we replaced URLs and user mentions with "URL" and "USER" strings. 











\section{Handling Imbalance Detest}



Table~\ref{tab:TaskData} highlights a significant imbalance in class distribution, particularly for \gls{ote} extraction. For instance, using \gls{ir} formula \ref{eq:IR}, the ratios for the majority class "O" and the minority classes "B-\gls{ote}" and "I-\gls{ote}" are found to be 10.11 and 52.03, respectively. Similarly, the IR for aspect sentiment classification between the majority (positive) and the minority (neutral) classes is 9.13. Such significant imbalances are known to adversely impact model performance, as documented in prior research \cite{imbalnceDSANDHandleit}.

We utilized focal loss along with class weights to mitigate this class imbalance. Focal Loss concentrates on misclassified or challenging examples by reducing the loss contribution from easily classified examples \cite{classImbalanceFocalLossPvsR}. At the same time, class weights recalibrate the loss based on class frequencies, giving more importance to minority classes.

We employed class weighting in conjunction with focal loss as our approach to addressing data imbalances. The class weights were computed using three distinct methods:

\begin{enumerate}
    \item \textbf{Imbalance Ratio (IR):} We calculated the IR as the ratio between the majority class $N_{\text{maj}}$ and each minority class $N_{\text{maj}}$ , yielding a whole integer representing the IR.
  \begin{equation}
    \text{IR} = \frac{N_{\text{min}}}{N_{\text{maj}}} \label{eq:IR}
    \end{equation}

    \item \textbf{Inverse Frequency Class Weighting:} The weights were computed using the formula:
    \begin{equation}
    w_j = \frac{N}{k \times n_j}
    \end{equation}
    \item \textbf{Inverse Frequency Class Weighting with Constant:} We further modified the weights by adding a constant and then normalizing:
    \begin{equation}
    w_j' = \frac{w_j + C}{\sum_{i=1}^{k} (w_i + C)}
    \end{equation}
\end{enumerate}

Where in the above formulas:
\begin{itemize}
    \item \( w_j \) and \( w_j' \) are the weights calculated for class \( j \).
    \item \( N \) is the total number of samples in the dataset.
    \item \( k \) represents the total number of distinct classes.
    \item \( n_j \) is the number of samples belonging to class \( j \).
    \item \( C \) is a constant added to each class weight in the latter method.
\end{itemize}




\section{Hyperparameter Settings}

We initially employed the Optuna library for hyperparameter selection, conducting 500 trials per model with feature extraction and full fine-tuning techniques. Optuna optimizes hyperparameters through Bayesian optimization using a Tree-structured Parzen Estimator\footnote{\url{https://optuna.org/}}~\citep{Akiba2019-Optuna}. For feature extraction, we froze all layers except the classification layer. The hyperparameters we considered included the learning rate, batch size, and number of epochs.


Due to computational constraints, each experiment with Optuna required 2-4 days, and some of the hyperparameters selected by Optuna resulted in suboptimal performance. Consequently, we investigated two alternative strategies: utilizing the default hyperparameters recommended for \gls{mbert}~\citep{devlin-etal-2019-bert} and employing task-specific hyperparameters used in Arabic pre-trained models for sequence and token classification tasks. For \gls{absa}, we utilized custom hyperparameters for sequence classification (e.g., sentence-level sentiment analysis). For \gls{ote}, we employed custom hyperparameters for token classification (e.g., named-entity recognition).

We compared the performance of models with Optuna-optimized hyperparameters to those using the default hyperparameters for \gls{mbert} and the task-specific hyperparameters from Arabic pre-trained models. Most models performed better with the default or task-specific hyperparameters, leading us to test \gls{ote} models with these settings only. Only three fully fine-tuned models showed marginally higher performance: Qarib by 0.2884\%, Arabic \gls{bert} by 0.1939\%, and CAMeLBERT-Mix by 0.1453\% in accuracy.

Tables~\ref{tab:hyeperparamters} and \ref{tab:OptunaHP} provide comprehensive details on the hyperparameter configuration and optimization process for various tested Arabic \gls{bert} models across different tasks (\gls{asc} and \gls{ote} extraction). Table~\ref{tab:hyeperparamters} includes details on whether full fine-tuning was applied, the learning rate, batch size, and number of epochs for each model. Table~\ref{tab:OptunaHP} presents the range of hyperparameters optimized via Optuna, including the learning rate, batch size, and number of epochs considered in the search process.



\input{HayperparamtersTABLE}

\input{OptunaHyperParamters}


For domain adaptation, we selected the three highest-performing models: CAMeLBERT-\gls{msa}, QARiB, and MARBERTV02. We continued pre-training these models using \gls{mlm} with a duplication factor of 10, whole-word masking at a 15\% rate, a batch size of 32, and a learning rate of 2.00E-05.

We used Optuna to determine the number of epochs by minimizing validation loss. To reduce the gap between dataset sizes, we considered a broader range of epochs for smaller datasets. We conducted experiments with each domain adaptation dataset for aspect sentiment classification and \gls{ote} extraction, using the \gls{hard} dataset for in-domain adaptation, the \gls{labr} dataset for out-of-domain adaptation, and \gls{semeval}-2016 Arabic hotel reviews training data for task adaptation. Table~\ref{tab:DAEPOCH} presents the epoch counts for domain-adapted models by dataset, listing each model with task-specific epochs.


\input{Number_of_epohcs_for_domain_adapted_modelsTL}

We selected CAMeLBERT-MSA as the base model for adapter domain adaptation due to its superior performance. We then continued pre-training it using a masked language model with a Pfeiffer invertible language adapter, a learning rate of 5.00E-05, and batch sizes of 64 and 128. To determine the optimal number of epochs, we evaluated accuracy and perplexity. Perplexity in \gls{mlm} measures a model's proficiency in accurately predicting masked tokens within a text sequence. Lower perplexity values indicate better predictive performance and a more robust understanding of the linguistic context. For the HARD dataset, we used 10\% of the data as the validation set, and for SemEval, we used 20\%.

Our results indicated that increasing the number of epochs improved accuracy and reduced perplexity. Thus, we used 50 epochs for in-domain adaptation with the \gls{hard} dataset and 400 epochs for the smaller \gls{semeval} dataset. Table~\ref{tab:AdapterLMHP} presents the hyperparameters and performance metrics for language model adapters across datasets, including perplexity, which is a language model performance metric where lower values indicate better performance.

We fine-tuned the adapters (task or language-task stacked) for 20 epochs with a batch size of 32 and a learning rate of 1e-4. For fused adapter models, we used the same settings except for a learning rate of 5e-5.

Following Focal Loss research guidelines, we explored gamma values from 1 to 5. Additionally, we tested class weights with constants varying from 0.1 to 0.9.




\input{AdaptersHPLM_TL}










==> OTEENLAPTOP.tex <==
\begin{table}[htp!]
\centering
\caption{Summary of Opinion Target Expression Extraction Techniques on SemEval-2014 English Laptop Reviews. Bold indicates the highest scores. Gains from domain adaptation are shown as percentages in parentheses (e.g., "\%1"). "N/A" indicates data not available.}
\label{tab:OTE_EN_LAP2014}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Reference} & \textbf{Year} & \textbf{Model} & \textbf{Word Embedding} & \textbf{Performance F1 (\%)} \\ \hline
\multicolumn{5}{|c|}{\textbf{LSTM+Attention}} \\ \hline 
\cite{ZschornackRodriguesSaraiva2021} & 2020 & \begin{tabular}[c]{@{}c@{}}POS-AttWD-\\ BLSTM-CRF\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pretrained \\ 300D-Glove\end{tabular} & 81.47 \\ \hline
\cite{Ma2020} & 2019 & Seq2Seq4ATE & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove,\\ Pretrained fastText\end{tabular} & 80.31 \\ \hline
\cite{Li2018} & 2018 & \begin{tabular}[c]{@{}c@{}}THA-STN\\ LSTMs\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pretrained \\ 300D-Glove\end{tabular} & 79.52 \\ \hline
\multicolumn{5}{|c|}{\textbf{CNN}} \\ \hline
\cite{Xu2018} & 2018 & DE-CNN & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove +\\ Domain-specific 100D-Fasttext\end{tabular} & 81.59 \\ \hline
\cite{Shu2019} & 2019 & Ctrl-CNN & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove +\\ Domain-specific 100D-Fasttext\end{tabular} & 82.73 \\ \hline
\cite{Ruidan2019} & 2019 & IMN & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove +\\ Domain-specific 100D-Fasttext\end{tabular} & 77.96 \\ \hline
\multicolumn{5}{|c|}{\textbf{BERT with Domain Adaptation}} \\ \hline
\cite{Xu2019} & 2019 & BERT-DK & Dom+BERT & 83.55 (+4.27) \\ \hline
\cite{Xu2019} & 2019 & PT-BERT & Dom+BERT & 84.26 \\ \hline
\cite{Xu2020c} & 2020 & DomBERT & Dom+BERT & 83.89 (+5.81) \\ \hline
\cite{YANG2021344} & 2020 & LCF-ATEPC-Fusion & Dom+BERT & 85.06 (+1.24) \\ \hline
\multicolumn{5}{|c|}{\textbf{BERT without Domain Adaptation}} \\ \hline
\cite{YANG2021344} & 2020 & LCF-ATEPC-Fusion & BERT & 83.82 \\ \hline
\cite{YANG2021344} & 2020 & LCF-ATE-CDM & BERT & 84.64 \\ \hline
\multicolumn{5}{|c|}{\textbf{Instruction-Tuning}} \\ \hline
\cite{Varia2022} & 2022 & \begin{tabular}[c]{@{}c@{}}Instruction-Tuning\\ Multi-task (IT-MTL)\\ T5\end{tabular} & T5 & 76.93 \\ \hline
\cite{scaria2023instructabsa} & 2023 & InstructABSA2 & Tk-Instruct & \textbf{92.30} \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> OTE_DA_table.tex <==
\begin{table*}[]
\caption{}
\label{tab:my-table}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{|ccccc|}
\hline
\multicolumn{5}{|c|}{\textbf{Camel-MSA}}                                                                                                                                                                         \\ \hline
\multicolumn{1}{|c|}{}              & \multicolumn{1}{c|}{Max}                       & \multicolumn{1}{c|}{avg}                      & \multicolumn{1}{c|}{var}                          & t-test                \\ \hline
\multicolumn{1}{|c|}{No-DAPT}       & \multicolumn{1}{c|}{F1:76.35,P:79.30,R:76.66}  & \multicolumn{1}{c|}{F1:76.20,P:77.88,R:74.65} & \multicolumn{1}{c|}{F1:0.0002,P:0.0351,R:0.0340}  &                       \\ \hline
\multicolumn{1}{|c|}{In-DAPT}       & \multicolumn{1}{c|}{F1:77.02,P:79.05,R:75.09}  & \multicolumn{1}{c|}{F1:76.47,P:78.46,R:74.58} & \multicolumn{1}{c|}{F1:0.0023,P:0.0048,R:0.0041}  & F1:0.45,P:0.73,R:0.95 \\ \hline
\multicolumn{1}{|c|}{Out-DAPT}      & \multicolumn{1}{c|}{F1:76.56,P:80.10,R:73.69}  & \multicolumn{1}{c|}{F1:76.22,P:79.53,R:73.18} & \multicolumn{1}{c|}{F1:0.0010,P:0.0048,R:0.0070}  & F1:0.93,P:0.30,R:0.20 \\ \hline
\multicolumn{1}{|c|}{TAPT}          & \multicolumn{1}{c|}{F1:76.48,P:78.41,R:75.86}  & \multicolumn{1}{c|}{F1:76.29,P:77.63,R:75.01} & \multicolumn{1}{c|}{F1:0.0006,P:0.0048,R:0.0056}  & F1:0.61,P:0.81,R:0.78 \\ \hline
\multicolumn{1}{|c|}{In-DAPT+TAPT}  & \multicolumn{1}{c|}{F1:76.43,P:79.09,R:74.36}  & \multicolumn{1}{c|}{F1:76.32,P:78.79,R:73.99} & \multicolumn{1}{c|}{F1:0.0001,P:0.0007,R:0.0013}  & F1:0.34,P:0.47,R:0.55 \\ \hline
\multicolumn{1}{|c|}{Out-DAPT+TAPT} & \multicolumn{1}{c|}{F1:76.40,P:76.35,R:76.92}  & \multicolumn{1}{c|}{F1:76.05,P:76.05,R:76.05} & \multicolumn{1}{c|}{F1:0.0011,P:0.0007,R:0.0076}  & F1:0.29,P:0.21,R:0.30 \\ \hline
\multicolumn{5}{|c|}{\textbf{QARiB}}                                                                                                                                                                             \\ \hline
\multicolumn{1}{|c|}{}              & \multicolumn{1}{c|}{Max}                       & \multicolumn{1}{c|}{avg}                      & \multicolumn{1}{c|}{var}                          & t-test                \\ \hline
\multicolumn{1}{|c|}{No-DAPT}       & \multicolumn{1}{c|}{F1:76.31,P:77.07,R:75.69}  & \multicolumn{1}{c|}{F1:76.09,P:76.78,R:75.41} & \multicolumn{1}{c|}{F1:0.0004,P:0.0015,R:0.0013}  &                       \\ \hline
\multicolumn{1}{|c|}{In-DAPT}       & \multicolumn{1}{c|}{F1:76.75,P:78.92,R:74.70}  & \multicolumn{1}{c|}{F1:76.47,P:78.58,R:74.46} & \multicolumn{1}{c|}{F1:0.0010,P:0.0020,R:0.0005}  & F1:0.06,P:0.00,R:0.04 \\ \hline
\multicolumn{1}{|c|}{Out-DAPT}      & \multicolumn{1}{c|}{F1:74.62,P:77.23,R:72.74}  & \multicolumn{1}{c|}{F1:74.13,P:76.19,R:72.19} & \multicolumn{1}{c|}{F1:0.0022,P:0.0167,R:0.0074}  & F1:0.01,P:0.38,R:0.01 \\ \hline
\multicolumn{1}{|c|}{TAPT}          & \multicolumn{1}{c|}{F1:76.45,P:78.04,R:75.80}  & \multicolumn{1}{c|}{F1:76.30,P:77.49,R:75.15} & \multicolumn{1}{c|}{F1:0.0004,P:0.0024,R: 0.0069} & F1:0.45,P:0.10,R:0.72 \\ \hline
\multicolumn{1}{|c|}{In-DAPT+TAPT}  & \multicolumn{1}{c|}{F1:76.79,P:78.75,R:75.26}  & \multicolumn{1}{c|}{F1:76.45,P:78.47,R:74.54} & \multicolumn{1}{c|}{F1:0.0009,P:0.0006,R:0.0040}  & F1:0.32,P:0.01,R:0.13 \\ \hline
\multicolumn{1}{|c|}{Out-DAPT+TAPT} & \multicolumn{1}{c|}{F1:70.27,P:75.80,R:71.48}  & \multicolumn{1}{c|}{F1:73.06,P:75.59,R:70.70} & \multicolumn{1}{c|}{F1:0.0024,P:0.0011,R:0.0095}  & F1:0.01,P:0.07,R:0.01 \\ \hline
\multicolumn{5}{|c|}{\textbf{MARBERTv2}}                                                                                                                                                                         \\ \hline
\multicolumn{1}{|c|}{}              & \multicolumn{1}{c|}{Max}                       & \multicolumn{1}{c|}{AVG}                      & \multicolumn{1}{c|}{VAR}                          & T-Test                \\ \hline
\multicolumn{1}{|c|}{No-DAPT}       & \multicolumn{1}{c|}{F1:76.64,P:77.36,R:78.82}  & \multicolumn{1}{c|}{F1:76.20,P:75.67,R:76.82} & \multicolumn{1}{c|}{F1:0.0037,P:0.0771,R:0.0306}  &                       \\ \hline
\multicolumn{1}{|c|}{In-DAPT}       & \multicolumn{1}{c|}{,F1:76.54,P:78.50,R:76.47} & \multicolumn{1}{c|}{F1:76.36,P:77.54,R:75.23} & \multicolumn{1}{c|}{F1:0.0005,P:0.0090,R:0.0119}  & F1:0.55,P:0.38,R:0.35 \\ \hline
\multicolumn{1}{|c|}{Out-DAPT}      & \multicolumn{1}{c|}{F1:74.44,P:75.00,R75.82}   & \multicolumn{1}{c|}{F1:74.04,P:74.07,R:74.04} & \multicolumn{1}{c|}{F1:0.0012,P:0.0090,R:0.0256}  & F1:0.06,P:0.29,R:0.00 \\ \hline
\multicolumn{1}{|c|}{TAPT}          & \multicolumn{1}{c|}{F1:76.59,P:77.45,R:75.75}  & \multicolumn{1}{c|}{F1:76.39,P:77.29,R:75.52} & \multicolumn{1}{c|}{F1:0.0003,P:0.0002,R:0.0005}  & F1:0.56,P:0.40,R:0.37 \\ \hline
\multicolumn{1}{|c|}{In-DAPT+TAPT}  & \multicolumn{1}{c|}{F1:76.95,P:78.63,R:77.53}  & \multicolumn{1}{c|}{F1:76.44,P:76.73,R:76.20} & \multicolumn{1}{c|}{F1:0.0022,P:0.0404,R:0.0135}  & F1:0.47,P:0.27,R:0.21 \\ \hline
\multicolumn{1}{|c|}{Out-DAPT+TAPT} & \multicolumn{1}{c|}{F1:75.76,P:76.85,R:74.98}  & \multicolumn{1}{c|}{F1:75.59,P:76.53,R:74.68} & \multicolumn{1}{c|}{F1:0.0002,P:0.0011,R:0.0011}  & F1:0.21,P:0.68,R:0.21 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}

==> OTE_EN_RES_2016_TL.tex <==
\begin{table}[htp!]
\centering
\caption{Summary of Opinion Target Extraction Techniques on SemEval-2016 English Restaurant Reviews. Bold indicates the highest scores. Gains from domain adaptation are shown as percentages in parentheses (e.g., "\%1"). "N/A" indicates data not available.}
\label{tab:OTE_EN_RES_16}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Reference} & \textbf{Year} & \textbf{Model} & \textbf{Word Embedding} & \textbf{Performance F1 (\%)} \\ \hline
\multicolumn{5}{|c|}{\textbf{LSTM+Attention}} \\ \hline
\cite{ZschornackRodriguesSaraiva2021} & 2020 & \begin{tabular}[c]{@{}c@{}}POS-AttWD-BLSTM-CRF\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove\end{tabular} & 73.04 \\ \hline
\cite{Ma2020} & 2019 & Seq2Seq4ATE & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove,\\ Pretrained fastText for OOV\end{tabular} & 75.14 \\ \hline
\cite{Li2018} & 2018 & THA-STN LSTMs & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove\end{tabular} & 73.61 \\ \hline
\multicolumn{5}{|c|}{\textbf{CNN}} \\ \hline
\cite{Xu2018} & 2018 & DE-CNN & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove +\\ Domain-specific 100D-Fasttext\end{tabular} & 74.37 \\ \hline
\cite{Shu2019} & 2019 & Ctrl-CNN & \begin{tabular}[c]{@{}c@{}}Pretrained 300D-Glove +\\ Domain-specific 100D-Fasttext\end{tabular} & 75.64 \\ \hline
\multicolumn{5}{|c|}{\textbf{BERT with Domain Adaptation}} \\ \hline
\cite{Xu2019} & 2019 & BERT-DK & \begin{tabular}[c]{@{}c@{}}Dom+BERT\end{tabular} & 77.02 (+2.92) \\ \hline
\cite{Xu2019} & 2019 & PT-BERT & \begin{tabular}[c]{@{}c@{}}Dom+BERT\end{tabular} & 77.97 \\ \hline
\cite{Xu2020c} & 2020 & DomBERT & \begin{tabular}[c]{@{}c@{}}Dom+BERT\end{tabular} & 77.21 (+4.20) \\ \hline
\multicolumn{5}{|c|}{\textbf{Instruction-Tuning}} \\ \hline
\cite{Varia2022} & 2022 & \begin{tabular}[c]{@{}c@{}}Instruction-Tuning\\ Multi-task Learning (IT-MTL)\end{tabular} & T5 & 79.41 \\ \hline
\cite{scaria2023instructabsa} & 2023 & InstructABSA1 & Tk-Instruct & \textbf{81.48} \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}




==> SP_DA_table.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|}
    \hline
        Camel-MSA & ~ & ~ & ~ & ~ \\ \hline
        ~ & Max & avg & var & t-test \\ \hline
        No-DAPT & acc:88.98,M-F1:73.72,M-P:78.74,M-R:73.50 & acc:87.92,M-F1:72.37,M-P:76.05,M-R:70.98 & acc:0.0093,M-F1:0.0246,M-P:0.0590,M-R:0.0636 & ~ \\ \hline
        In-DAPT & acc:89.17,M-F1:75.62,M-P:78.52,M-R:76.16 & acc:88.91,M-F1:75.56,M-P:77.16,M-R:74.66 & acc:0.0017,M-F1:0.0001,M-P:0.0321,M-R:0.0170 & acc:0.21,M-F1:0.07,M-P:0.44,M-R:0.05 \\ \hline
        Out-DAPT & acc:87.63,M-F1:73.39,M-P:76.22,M-R:73.09 & acc:87.15,M-F1:67.19,M-P:73.57,M-R:67.09 & acc:0.0043,M-F1:0.2886,M-P:0.0754,M-R:0.2715 & acc:0.49,M-F1:0.17,M-P:0.47,M-R:0.16 \\ \hline
        TAPT & acc:87.86,M-F1:67.66,M-P:76.29,M-R:66.21 & acc:87.29,M-F1:64.28,M-P:74.56,M-R:64.24 & acc:0.0028,M-F1:0.1483,M-P:0.0272,M-R:0.0453 & acc:0.54,M-F1:0.07,M-P:0.43,M-R:0.05 \\ \hline
        In-DAPT+TAPT & acc:87.75,M-F1:74.34,M-P:74.26,M-R:74.47 & acc:87.43,M-F1:71.35,M-P:73.69,M-R:70.56 & acc:0.0012,M-F1:0.0880,M-P:0.0089,M-R:0.1250 & acc:0.59,M-F1:0.60,M-P:0.35,M-R:0.81 \\ \hline
        Out-DAPT+TAPT & acc:87.14,M-F1:71.98,M-P:74.96,M-R:71.48 & acc:86.83,M-F1:66.48,M-P:72.92,M-R:66.15 & acc:0.0008,M-F1:0.2284,M-P:0.0364,M-R:0.2139 & acc:0.11,M-F1:0.12,M-P:0.30,M-R:0.09 \\ \hline
        QARiB & ~ & ~ & ~ & ~ \\ \hline
        ~ & Max & avg & var & t-test \\ \hline
        No-DAPT & acc:86.83,M-F1:71.69,M-P:75.12,M-R:71.03 & acc:86.58,M-F1:64.94,M-P:71.28,M-R:65.26 & acc:0.0009,M-F1:0.3700,M-P:0.2164,M-R:0.2667 & ~ \\ \hline
        In-DAPT & acc:88.29,M-F1:70.61,M-P:75.95,M-R:69.47 & acc:87.17,M-F1:65.39,M-P:72.18,M-R:65.47 & acc:0.0095,M-F1:0.2117,M-P:0.1736,M-R:0.1215 & acc:0.37,M-F1:0.81,M-P:0.15,M-R:0.89 \\ \hline
        Out-DAPT & acc:85.29,M-F1:69.74,M-P:69.59,M-R:69.91 & acc:84.90,M-F1:66.40,M-P:67.91,M-R:66.34 & acc:0.0039,M-F1:0.1272,M-P:0.0213,M-R:0.1517 & acc:0.01,M-F1:0.49,M-P:0.31,M-R:0.48 \\ \hline
        TAPT & acc:86.83,M-F1:72.29,M-P:72.56,M-R:72.17 & acc:86.33,M-F1:68.71,M-P:70.40,M-R:68.86 & acc:0.0035,M-F1:0.2678,M-P:0.0654,M-R: 0.2566 & acc:0.66,M-F1:0.31,M-P:0.85,M-R:0.29 \\ \hline
        In-DAPT+TAPT & acc:87.21,M-F1:70.62,M-P:72.87,M-R:69.62 & acc:86.76,M-F1:64.91,M-P:71.27,M-R:65.10 & acc:0.0017,M-F1:0.2491,M-P:0.0447,M-R:0.1536 & acc:0.51,M-F1:1.00,M-P:1.00,M-R:0.98 \\ \hline
        Out-DAPT+TAPT & acc:86.52,M-F1:70.27,M-P:74.63,M-R:70.53 & acc:84.28,M-F1:66.01,M-P:70.17,M-R:66.84 & acc:0.0630,M-F1:0.2039,M-P:0.1933,M-R:0.1919 & acc:0.22,M-F1:0.51,M-P:0.27,M-R:0.39 \\ \hline
        MARBERTv2 & ~ & ~ & ~ & ~ \\ \hline
        ~ & Max & avg & var & t-test \\ \hline
        No-DAPT & acc:87.40,M-F1:,M-P:70.76,M-R:67.34 & acc:87.12,M-F1:67.65,M-P:69.63,M-R:65.48 & acc:0.0008,M-F1:0.0413,M-P:0.0157,M-R:0.0275 & ~ \\ \hline
        In-DAPT & acc:87.94,M-F1:,M-P:73.04,M-R:71.95 & acc:87.39,M-F1:70.07,M-P:72.62,M-R:70.67 & acc:0.0025,M-F1:0.0068,M-P:0.0030,M-R:0.0127 & acc:0.18,M-F1:0.07,M-P:0.09,M-R:0.07 \\ \hline
        Out-DAPT & acc:87.25,M-F1:,M-P:71.72,M-R:67.55 & acc:86.93,M-F1:68.50,M-P:70.61,M-R:66.85 & acc:0.0016,M-F1:0.0132,M-P:0.0170,M-R:0.0126 & acc:0.34,M-F1:0.48,M-P:0.18,M-R:0.48 \\ \hline
        TAPT & acc:86.90,M-F1:,M-P:71.97,M-R:66.35 & acc:86.75,M-F1:67.48,M-P:69.34,M-R:64.78 & acc:0.0002,M-F1:0.0505,M-P:0.0592,M-R:0.0199 & acc:0.25,M-F1:0.29,M-P:0.83,M-R:0.28 \\ \hline
        In-DAPT+TAPT & acc:87.52,M-F1:,M-P:73.08,M-R:67.96 & acc:87.35,M-F1:68.46,M-P:71.43,M-R:66.42 & acc:0.0002,M-F1:0.0808,M-P:0.0356,M-R:0.0448 & acc:0.23,M-F1:0.73,M-P:0.42,M-R:0.71 \\ \hline
        Out-DAPT+TAPT & acc:87.10,M-F1:,M-P:68.32,M-R:65.18 & acc:86.73,M-F1:66.71,M-P:67.69,M-R:64.30 & acc:0.0021,M-F1:0.0149,M-P:0.0112,M-R:0.0068 & acc:0.38,M-F1:0.37,M-P:0.20,M-R:0.43 \\ \hline
    \end{tabular}
    \caption{Aspect-Sentiment Classification (sentence pair input)}
\end{table}

==> SemEval2014ENtable.tex <==
\begin{table}[htp!]
\centering
\caption{Summary of SemEval-2014 Laptop and Restaurant English Datasets.}
\label{tab:SemEval2014DS}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Format} & \multirow{2}{*}{Training} & \multirow{2}{*}{Testing} & \multirow{2}{*}{Total} & \multicolumn{2}{c|}{\#Aspect terms} & \multirow{2}{*}{Balanced} & \multirow{2}{*}{ID} \\ \cline{6-7}
                         &                         &                           &                          &                        & Train & Test &                           &                           \\ \hline
\begin{tabular}[c]{@{}c@{}}Restaurant Reviews\\ -2014\\ \cite{Pontiki2014}\end{tabular} & SemEval-2014 & \begin{tabular}[c]{@{}c@{}}3041\\ Sentences\end{tabular} & \begin{tabular}[c]{@{}c@{}}800\\ Sentences\end{tabular} & 3841 & 2358 & 654 & No & ED1 \\ \hline
\begin{tabular}[c]{@{}c@{}}Laptop Reviews\\ -2014\\ \cite{Pontiki2014}\end{tabular} & SemEval-2014 & \begin{tabular}[c]{@{}c@{}}3045\\ Sentences\end{tabular} & \begin{tabular}[c]{@{}c@{}}800\\ Sentences\end{tabular} & 3845 & 3693 & 1134 & No & ED2 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> StackedLMSTL.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Stacked language models  }
\label{tab:StackedLM}
\begin{adjustbox}{width=\textwidth, center}
\begin{tabular}{
    >{\centering\arraybackslash}p{0.3\textwidth}
    >{\centering\arraybackslash}p{0.3\textwidth}
    >{\centering\arraybackslash}p{0.3\textwidth}
    >{\centering\arraybackslash}p{0.3\textwidth}
}
\toprule
Max(\%)&
  Average(\%) &
  Variance(\%) &
  P-value \\ \midrule
\multicolumn{4}{c}{\textbf{Opinion Target Extraction}} \\ \midrule
\multicolumn{4}{c}{CAMeLBERT-MSA-QARiB-DAPT(HARD)} \\ \midrule
F1:76.14,P:76.85,
R:78.96 &
  F1:76.01,P:75.24,
  R:76.84 &
  F1:0.0003,P:0.0280,
  R:0.0361 &
  F1:0.37,P:0.01,
  R:0.00 \\ \midrule
\multicolumn{4}{c}{CAMeLBERT-MSA-QARiB-DAPT(HARD)-MARBERTv2-DAPT+TAPT(HARD+SemEval)} \\ \midrule
F1:\textbf{76.45},P:74.65,
R:78.33 &
  F1\textbf{:76.13},P:74.17,
  R:78.20 &
  F1:0.0015,P0.0059,
  R:0.0003 &
  F1:0.83,P:0.11
  ,R:0.07 \\ \midrule
\multicolumn{4}{c}{CAMeLBERT-MSA-DAPT(HARD)-TAPT(SemEval)-DAPT+TAPT(HARD+SemEval)} \\ \midrule
F1:76.39,P:74.88,
R:79.17 &
  F1:75.99,P:74.07,
  R:78.04 &
  F1:0.0017,P:0.0050,
  R:0.0242 &
  F1:0.59,P:0.06,
  R:0.13 \\ \midrule
\multicolumn{4}{c}{\textbf{Aspect-sentiment classification sentence-pair}} \\ \midrule
\multicolumn{4}{c}{CAMeLBERT-MSA-MARBERTv2-DAPT(HARD)} \\ \midrule
acc:\textbf{89.78},M-F1:77.35,M-P:78.00,M-R:76.77 &
  acc:\textbf{89.53},M-F:173.94,M-P:76.91,M-R:73.19 &
  acc:0.0012,M-F1:0.3226,M-P:0.0329,M-R:0.3430 &
  acc:0.07,M-F1:0.59,M-P:0.63,M-R:0.43 \\ \midrule
\multicolumn{4}{c}{CAMeLBERT-MSA-MARBERTV02-QARiB-DAPT(HARD)} \\ \midrule
acc:89.25,M-F1:76.44,
M-P:77.88,M-R:75.89&
  acc:88.43,M-F1:72.20,
  M-P:73.80,M-R:71.24 &
  acc:0.0084,M-F1:0.2077,
  M-P:0.4080,M-R:0.1859 &
  acc:0.46,M-F1:0.93,
  M-P:0.59,M-R:0.83 \\ \midrule
\multicolumn{4}{c}{CAMeLBERT-MSA-DAPT(HARD)-TAPT(SemEval)-DAPT+TAPT(HARD+SemEval)} \\ \midrule
acc:87.83,M-F1:71.56,
M-P:79.42,M-R:71.71 &
  acc:87.34,M-F1:66.06,
  M-P:76.43,M-R:66.46 &
  acc:0.0047,M-F1:0.2415,
  M-P:0.1855,M-R:0.2141 &
  acc:0.60,M-F1:0.13,
  M-P:0.93,M-R:0.25 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
